Hybrid Metabolic Network Completion

Metabolic networks play a crucial role in biology since they capture all chemical reactions in an organism. While there are networks of high quality for many model organisms, networks for less studied organisms are often of poor quality and suffer from incompleteness. To this end, we introduced in previous work an ASP-based approach to metabolic network completion. Although this qualitative approach allows for restoring moderately degraded networks, it fails to restore highly degraded ones. This is because it ignores quantitative constraints capturing reaction rates. To address this problem, we propose a hybrid approach to metabolic network completion that integrates our qualitative ASP approach with quantitative means for capturing reaction rates. We begin by formally reconciling existing stoichiometric and topological approaches to network completion in a unified formalism. With it, we develop a hybrid ASP encoding and rely upon the theory reasoning capacities of the ASP system clingo for solving the resulting logic program with linear constraints over reals. We empirically evaluate our approach by means of the metabolic network of Escherichia coli. Our analysis shows that our novel approach yields greatly superior results than obtainable from purely qualitative or quantitative approaches. Under consideration in Theory and Practice of Logic Programming (TPLP).

==> bbl.tex <==
\begin{thebibliography}{10}

% \bibitem{Acuna2009}
% V.~Acu{\~{n}}a, F.~Chierichetti, V.~Lacroix, A.~Marchetti-Spaccamela, M.~Sagot, L.~Stougie.
% \newblock {Modes and cuts in metabolic networks: Complexity and algorithms}.
% \newblock {\em Biosystems}, 95(1):51--60, 2009.

\bibitem{anbole13a}
C.~Ans{\'o}tegui, M.~Bonet, J.~Levy.
\newblock {SAT}-based {MaxSAT} algorithms.
\newblock {\em Artificial Intelligence}, 196:77--105, 2013.

\bibitem{baral02a}
C.~Baral.
\newblock {\em Knowledge Representation, Reasoning and Declarative Problem Solving}.
\newblock Cambridge, 2003.

\bibitem{Becker2007}
S.~Becker, A.~Feist, M.~Mo, G.~Hannum, B.~Palsson, M.~Herrgard.
\newblock {Quantitative Prediction of Cellular Metabolism with Constraint-based Models: The COBRA Toolbox}.
\newblock {\em Nature Protocols}, 2(3):727--738, 2007.

\bibitem{coevgeprscsith13a}
G.~Collet, D.~Eveillard, M.~Gebser, S.~Prigent, T.~Schaub, A.~Siegel, S.~Thiele.
\newblock Extending the metabolic network of {E}ctocarpus siliculosus using answer set programming.
\newblock 
% In P.~Cabalar and T.~Son, editors, {\em Proceedings of the Twelfth International Conference on Logic Programming and Nonmonotonic Reasoning (LPNMR'13)}, volume 8148 of {\em Lecture Notes in Artificial Intelligence}, 
{\em Proceedings LPNMR},
245--256. Springer, 2013.

\bibitem{dantzig63a}
G.~Dantzig.
\newblock {\em Linear Programming and Extensions}.
\newblock Princeton, 1963.

% \bibitem{ebhahe04a}
% O.~Ebenhöh, T.~Handorf, R.~Heinrich.
% \newblock Structural analysis of expanding metabolic networks.
% \newblock {\em Genome Informatics}, 15(1):35--45, 2004.

\bibitem{Ebrahim2013}
A.~Ebrahim, J.~Lerman, B.~Palsson, D.~Hyduke.
\newblock {COBRApy: COnstraints-Based Reconstruction and Analysis for Python.}
\newblock {\em BMC Systems Biology}, 7:74, aug 2013.

\bibitem{gekakaosscwa16a}
M.~Gebser, R.~Kaminski, B.~Kaufmann, M.~Ostrowski, T.~Schaub, P.~Wanko.
\newblock Theory solving made easy with clingo~5.
\newblock 
% In M.~Carro and A.~King, editors, {\em Technical Communications of the Thirty-second International Conference on Logic Programming (ICLP'16)}, volume~52, 
{\em Technical Comm.\ ICLP},
2:1--2:15. 
% Open Access Series in Informatics
OASIcs, 2016.

\bibitem{gekakarosc15a}
M.~Gebser, R.~Kaminski, B.~Kaufmann, J.~Romero, T.~Schaub.
\newblock Progress in clasp series 3.
\newblock 
% In F.~Calimeri, G.~Ianni, and M.~Truszczy{\'n}ski, editors, {\em Proceedings of the Thirteenth International Conference on Logic Programming and Nonmonotonic Reasoning (LPNMR'15)}, volume 9345 of {\em Lecture Notes in Artificial Intelligence}, 
{\em Proceedings LPNMR},
368--383. Springer, 2015.

\bibitem{gellif91a}
M.~Gelfond, V.~Lifschitz.
\newblock Classical negation in logic programs and disjunctive databases.
\newblock {\em New Generation Computing}, 9:365--385, 1991.

\bibitem{haebhe05a}
T.~Handorf, O.~Ebenhöh, R.~Heinrich.
\newblock Expanding metabolic networks: Scopes of compounds, robustness, and evolution.
\newblock {\em J.\ of Molec.\ Evolution}, 61(4):498--512, 2005.

\bibitem{laten2014a}
M.~Latendresse.
\newblock Efficiently gap-filling reaction networks.
\newblock {\em BMC bioinformatics}, 15(1):225, 2014.

\bibitem{marzom16a}
C.~Maranas, A.~Zomorrodi.
\newblock {\em Optimiz.\ methods in metabolic networks}.
\newblock Wiley, 2016.

\bibitem{Orth2010}
J.~Orth, B.~Palsson.
\newblock {Systematizing the generation of missing metabolic knowledge.}
\newblock {\em Biotechnology and bioengineering}, 107(3):403--12, oct 2010.

% \bibitem{orthpa10a}
% J.~Orth, I.~Thiele, B.~Palsson.
% \newblock What is flux balance analysis?
% \newblock {\em Nature biotechnology}, 28(3):245--248, 2010.

\bibitem{ostsch12a}
M.~Ostrowski, T.~Schaub.
\newblock {ASP} modulo {CSP}: The clingcon system.
\newblock {\em Theory and Practice of Logic Programming}, 12(4-5):485--503, 2012.

% \bibitem{potassco}
% Potassco website.
% \newblock http://potassco.org.

\bibitem{prcodideetdaevthcabosito14a}
S.~Prigent, G.~Collet, S.~Dittami, L.~Delage, F.~{Ethis de Corny}, O.~Dameron, D.~Eveillard, S.~Thiele, J.~Cambefort, C.~Boyen, A.~Siegel, T.~Tonon.
\newblock The genome-scale metabolic network of ectocarpus siliculosus (ectogem): a resource to study brown algal physiology and beyond.
\newblock {\em The Plant Journal}, 80(2):367–381, 2014.

\bibitem{Prigent2017}
S.~Prigent, C~.Frioux, S.~Dittami, S.~Thiele, A.~Larhlimi, G.~Collet, F.~Gutknecht, J.~Got, D.~Eveillard, J.~Bourdon, F.~Plewniak, T.~Tonon, A.~Siegel.
\newblock {Meneco, a Topology-Based Gap-Filling Tool Applicable to Degraded Genome-Wide Metabolic Networks}.
\newblock {\em PLOS Computational Biology}, 13(1):e1005276, jan 2017.

\bibitem{Reed2003}
J.~Reed, T.~Vo, C.~Schilling, B.~Palsson.
\newblock {An expanded genome-scale model of Escherichia coli K-12 (iJR904 GSM/GPR).}
\newblock {\em Genome Biology}, 4(9):R54, 2003.

\bibitem{SatishKumar2007}
V.~{Satish Kumar}, M.~Dasika, C.~Maranas.
\newblock {Optimization based automated curation of metabolic reconstructions}.
\newblock {\em BMC Bioinformatics}, 8(1):212, 2007.

\bibitem{schthi09a}
T.~Schaub, S.~Thiele.
\newblock Metabolic network expansion with {ASP}.
\newblock
% In P.~Hill and D.~Warren, editors, {\em Proceedings of the Twenty-fifth International Conference on Logic Programming (ICLP'09)}, volume 5649 of {\em Lecture Notes in Computer Science}, 
{\em Proceedings ICLP},
312--326. Springer, 2009.

\bibitem{siniso02a}
P.~Simons, I.~Niemelä, T.~Soininen.
\newblock Extending and implementing the stable model semantics.
\newblock {\em Artificial Intelligence}, 138(1-2):181--234, 2002.

\bibitem{Thiele2014}
I.~Thiele, N.~Vlassis, R.~Fleming.
\newblock {fastGapFill: efficient gap filling in metabolic networks.}
\newblock {\em Bioinformatics}, 30(17):2529--2531, sep 2014.

\bibitem{Vitkin2012}
E.~Vitkin, T.~Shlomi.
\newblock {MIRAGE: a functional genomics-based approach for metabolic network model reconstruction and its application to cyanobacteria networks.}
\newblock {\em Genome Biology}, 13(11):R111, 2012.

\end{thebibliography}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> problem2.tex <==
%!TEX root = paper.tex

\section{Metabolic Network Completion}\label{sec:problem}

%
Metabolism is the sum of all chemical reactions occurring within an organism. 
%
As the products of a reaction may be reused as reactants, reactions can be chained to complex chemical pathways.
%
Such complex pathways are described by a metabolic network.

%
A \emph{metabolic network} is commonly represented as a directed bipartite graph
\(
(R\cup M,E),
\)
where $R$ and $M$ are sets of nodes standing for \emph{reactions} and \emph{metabolites}, respectively.
%
When $(m,r)\in E$ or $(r,m)\in E$ for $m\in M$ and $r\in R$, the metabolite $m$ is called a \emph{reactant} or \emph{product} of reaction~$r$, respectively.
%
More formally, for any $r\in R$, define
\(
\Reactants{r}=\{m\in M\mid (m,r)\in E\}
\)
and
\(
\Products{r} =\{m\in M\mid (r,m)\in E\}
\).

%
Quantitatively, reactions are subject to \emph{stoichiometry} for balancing the relative quantities of reactants and products.
%
This can be captured by an \emph{edge labeling} giving the stoichiometric coefficient of a reaction's reactants and products, viz.\
\(
\StoichiometricFunction: E\rightarrow \mathbb{Q}
\),
respectively.
%
We call
\(
(R\cup M,E,\StoichiometricFunction)
\)
a \emph{stoichiometric metabolic network}. 
%
In addition, the activity rate of reactions $r\in R$ is bounded by lower bound $\MinFlux{r}=0$ and upper bound $\MaxFlux{r}\in\mathbb{R}^+$, respectively.

%
We introduce the notation $S \subseteq M$ to model {\em initiation seeds}, a set of metabolic compounds which are assumed to be present in the system at its initial state
due to data gathered in an experimental setup.
%
In addition, the graph structure carries out a specific set of compounds whose production is intrinsically assumed to be activated by default. These {\em boundary compounds} are defined as follows:
\(
 \strseed(G) = \{ m\in M \, | \,  m\in \Products{r}, \Reactants{r}=\emptyset \} \subseteq M
\).
% 
For the sake of clarity, in the network completion problem described in the paper, we will assume that all boundary compounds are seeds: $\strseed(G) \subset S$. Notice, however, that the concepts of reachability and activity on which the network completion problem is based are more generic and independent of this assumption.

%This corresponds to the set of metabolic compounds whose production is assumed to be activated by external control. 
%Let $S=\strseed(G)\cup\initseed$ denote the union of all seeds of the metabolic network.

%
For illustration, consider the stoichiometric metabolic network in Fig.~\ref{gra:toy} and ignore the shaded part. 
%
% ----------------------------------------------------------------------
\begin{figure}[ht]
  \centering
    \input{toypic}
    \caption{Example of a metabolic network}
    \label{gra:toy}
\end{figure}
% ----------------------------------------------------------------------
%
The network consists of 6 reactions, $r_{inS}$, $r_{expF}$ and $r_0$ to $r_5$, and 8 metabolites, $A,\dots,F$, $S_1$, $S_2$.
Here, $S=\{S_1,S_2\}$, $S_1$ being the only boundary compound of the network.
%
Consider reaction
\(
r_4 : E\rightarrow 2C
\)
transforming one unit of $E$ into two units of $C$.
%
We have
$\Reactants{r_4}=\{E\}$,
$\Products{r_4}=\{C\}$,
along with $\Stoichiometry{E}{r_4}=1$\footnote{Stoichiometric coefficients of 1 are omitted in the graphical representation; cf.~Fig.\ref{gra:toy}.}
and $\Stoichiometry{r_4}{C}=2$.


%
In the applicative domain of biology, several concepts have been introduced to model the capability of a metabolic network to  activate  flux reactions, or, equivalently, to  synthesize metabolic compounds.
%
We hereby assume that the capability of a stoichiometric metabolic network $G$ to activate a set of reaction fluxes
can be modeled by a function $\Reachability$ taking as input any set of seeds $S \subseteq M$, that consists of initial and/or boundary seeds as described above,
and having as output a set of activated reactions $\Reachability(G,S) \subseteq R$. 
%
In this setting, the {\em metabolic network completion problem} aims at ensuring that a set of targeted reactions is activated from the seed compounds $S$, 
possibly by adding to the metabolic network additional reactions picked up in a reference network (shaded part of the network in ~Fig.\ref{gra:toy}).

% 
 Formally, we assume that we are given a stoichiometric metabolic network $G=(R\cup M,E,\mathit{stc})$ with its bounds, 
 a set of seed metabolites $S$ with the property that $\strseed(G) \subset S$, 
 a set of targeted reactions $R_{T}\subseteq R$ and a reference network $(R'\cup M',E',\mathit{stc}')$.
 %
The \emph{metabolic network completion problem} is to find a set $R''\subseteq R'\setminus R$ of reactions with minimal size such that
\(
R_{T}\subseteq\Reachability(G'',S)
\),
where
\begin{align}
\label{eq:completion:graph}
  G''&= ((R\cup R'')\cup (M\cup M''),E\cup E'',\mathit{stc}'')\ ,
\\\label{eq:completion:metabolites}
M''&=\{m\in M'\mid r\in R'', m\in\Reactants{r}\cup\Products{r}\}\ , 
\\\label{eq:completion:edges}
E''&=E'\cap((M''\times R'')\cup(R''\times M'')) , \text{ and}
\\
\mathit{stc}''&=\mathit{stc}\cup\mathit{stc}'
\ .
\end{align}
%
We call $R''$ a \emph{completion} of $(R\cup M,E,\mathit{stc})$ from $(R'\cup M',E',\mathit{stc}')$ 
wrt $S$ and $R_{T}$.
%
Further refinements may also be interested in subset-minimal completions or optimize the distance between seeds and targets or minimize forbidden side products (cf.~\cite{schthi09a}).

%
The concept of activated reactions $\Reachability$ can be modeled differently according to different paradigms introduced in biology.
%
Therefore, there are several different metabolic network completion problem formulations: the stoichiometric, the relaxed stoichiometric, the topological, and the hybrid one. %
They are formally defined in the following sections.

\subsection{Stoichiometric Metabolic Network Completion}
\label{sec:stoichio}

The first semantics associated to the concept of activated reactions has been introduced in the context of Flux Balance Analysis (FBA) \cite{Orth2010}, 
a linear-algebra paradigm allowing for modeling and studying reaction flux distributions of stoichiometric metabolic networks at steady-state.
%
In this paradigm, each reaction $r$ is associated with a \emph{metabolic flux value} $v_r$, a real variable confined by the maximum rates \MaxFlux{r}
%
\begin{align} \label{eq:stoichiometric:bounds}
   & \MinFlux{r} \leq  v_r\leq \MaxFlux{r}
                       \qquad\text{ for } r\in R 
\end{align}
% 
\comment{C: lb or 0 in (5) ?}
Flux distributions are formalized in terms of a system of equations relying on the stoichiometric coefficients of reactions.
%
Reaction rates are governed by the \emph{law of mass conservation} which assumes a steady state, that is, the input and output rates of reactions consuming and producing a metabolite are balanced.
%
\begin{align}  
\label{eq:stoichiometric:equation}
  &  \textstyle
                       \sum_{\substack{r\in R}}\Stoichiometry{r}{m}\cdot v_r
                       +
                       \sum_{\substack{r\in R}}-\Stoichiometry{m}{r}\cdot v_r
                       =
                       0
                       \quad \text{ for } m\in M   
\end{align}
%
%Equations \eqref{eq:stoichiometric:bounds} and \eqref{eq:stoichiometric:equation} are part of the Flux Balance Analysis (FBA) framework \cite{Orth2010} that aims to optimize flux in a target reaction.
Given a reaction $r_T\in R_T$, a stoichiometric metabolic network $(R\cup M,E,\mathit{stc})$ and a set of seeds $S$,
{\em stoichiometrically activated} is defined as follows: 
  \begin{align}   \label{eq:stoichiometric:objective}  
   r_T \in \Reachability^{(st)} (S) & \iff \forall r \in R, \, \exists  v_r \geq 0 \mbox{ s.t.  Eqs.}~\eqref{eq:stoichiometric:bounds},\eqref{eq:stoichiometric:equation}\mbox{ hold and } v_{r_T} >0.
      \end{align} 
We shall notice that from this definition, activated target reactions do not depend directly on the set of seeds $S$ of the network.  \comment{C: Changed S by Sinit because Sbdr are attributes of G and are thus taken into account here}
On the other hand, activated targets reactions highly depend of boundary compounds from $\strseed$ for which \eqref{eq:stoichiometric:equation} is always satisfied and allows to initiate the values of fluxes.
%

In practice, the database can be insufficient to restore the steady-state criteria depicted by equation \eqref{eq:stoichiometric:equation}. 
%
This can be circumvented by enabling the creation of so called \sysfont{export} reactions to balance the amount of compounds that cannot be balanced with existing reactions in the draft or the database.
We see such export reaction in Figure~\ref{gra:toy} for compound $F$. 

%

To solve the {\em stoichiometric completion} based on flux-balance activated reactions, 
Linear Programming (LP)~\cite{dantzig63a} can be used to maximize the flux rate $v_{r_T}$ under the hypothesis that the linear constraints are satisfied.
%
In practice, this problem is intractable. 
%
The relaxed problem consists in relaxing the mass-balance equation  \eqref{eq:stoichiometric:equation} as follows:
%
\begin{align}  
\label{eq:stoichiometric:equation:relaxed}
  &  \textstyle
                       \sum_{\substack{r\in R}}\Stoichiometry{r}{m}\cdot v_r
                       +
                       \sum_{\substack{r\in R}}-\Stoichiometry{m}{r}\cdot v_r
                       \geq 
                       0
                       \quad \text{ for } m\in M    
\end{align}
%
The {\em relaxed stoichiometric completion problem} is based on the following semantics for activated reactions:
  \begin{align*}   
   r_T \in \Reachability^{(strl)} (G,S) & \iff \forall r \in R, \, \exists  v_r \geq 0 \mbox{ s.t.  Eqs.}~\eqref{eq:stoichiometric:bounds},\eqref{eq:stoichiometric:equation:relaxed}\mbox{ hold and } v_{r_T} >0.
      \end{align*}
This problem can be efficiently solved with LP \cite{SatishKumar2007}.  
%
Notice however that, when interested in strict steady-state modeling (FBA), an \textit{a posteriori} verification of the output solution is needed to check whether equation \eqref{eq:stoichiometric:equation} is satisfied. 

In the example network, $G$ consisting of all bold nodes and edges depicted in Figure \ref{gra:toy}. A strict stoichiometry-based completion \comment{C: removed FBA-based, seemed unclear} aims to obtain a positive value when maximizing the flux in $r_{5}$. 
%
This can be achieved by adding the set of reactions $\{r_{6},r_9\}$. 
%
The cycle made of compounds $E,C,D$ is already balanced and self-activated.
%
The instance of equation~\eqref{eq:stoichiometric:equation} controlling the reaction rates related to metabolite $C$ is
\(
2\cdot v_{r_4} - v_{r_2} - v_{r_5} = 0
\).

%
While we are not aware of implementations of the stoichiometric completion problem using Equation~\eqref{eq:stoichiometric:equation},
the system \gapfill~\cite{SatishKumar2007} solves the relaxed problem~\eqref{eq:stoichiometric:equation:relaxed}.

\subsection{Topological Metabolic Network Completion}
\label{sec:topo}

%
In the topological metabolic network completion problem, the semantics associated to the activation of reactions is based on the study of the graph topology.
%
Given a metabolic network $G$, a reaction $r\in R$ is \emph{activated} from a set of seeds $S$ if all reactants in $\Reactants{r}$ are reachable from~$S$.
%
Moreover, a metabolite $m\in M$ is \emph{reachable} from $S$ if %
$m\in S$
or if
$m\in\Products{r}$ for some reaction $r\in R$ where all $m'\in\Reactants{r}$ are reachable from~$S$.
%
The \emph{scope} of $S$, written $\Sigma(G,S)$, is the closure of metabolites reachable from~$S$. 
%
In this setting, \emph{topological activation} of reactions from a set of seeds $S$ is defined as follows:  
%
  \begin{align*}   
   r_T \in \Reachability^{(top)}(G,S) \iff \forall m \in \Reactants{r_T}\mbox{ holds }m \in \Sigma(G,S).   \label{eq:topological}
  \end{align*}
%
The {\em topological completion} problem, based of this topological notion of activation of reactions, is a combinatorial optimization problem. 
%
It amounts to a simple form of abductive reasoning. 


For illustration, consider the metabolic network $G$ consisting of all bold nodes and edges in Fig.~\ref{gra:toy}, 
viz.\ reactions $r_1$ to $r_5$, $r_{inS}$ and metabolites $A,\dots,F$, $S_1$ and $S_2$, the latter being a initiation metabolite and $r_5$ the single target reaction.
%
We get $\Sigma_{G}(\{S_1,S_2\})=\{S_1,S_2,B\}$, which indicates that the target reaction $r_5$ is not activated from the seed with the current network
because $A$ and $C$ are not reachable.
%
This changes once the network is completed.
%
Valid minimal completions are $R''_1=\{r_6,r_7\}$ and $R''_2=\{r_6,r_8\}$ \comment{C: removed , and $R''_3=\{r_6,r_7,r_8\}$ because in problem def we say minimal size} because
\(
r_5\in\Reachability{(top)}(G_i,\{S_1,S_2\})\mbox{ since }\{A,C\}\subseteq\Sigma_{G}(\{S_1,S_2\})
\)
for all extended networks $G_i$ obtained from completions $R''_i$ of $G$ for $i=\{1,2\}$ \comment{removed $1,\dots,3 $for the same reason}.
%
Relevant elements from the reference network are given in dashed gray.


\subsection{Hybrid Metabolic Network Completion}
\label{sec:hybrid}

The idea of hybrid metabolic network completion is to combine the two previous semantics: 
the topological one that takes into account the initiation of the system, 
and the stoichiometric one that models the steady state.
% 
This means that we aim to compute network completions that are both topologically functional and flux balanced (without suffering from self-activated cycles\comment{T: Issue to be introduced above. A: I do not know wether we have space to explain this question of cycles}).
%
To formalize this setting, we introduce the {\em hybrid} semantics for activation as follows. 
%
A reaction $r\in R_T$ is {\em hybrid activated} from a set of seeds $S$ if it both stoichiometric and topological activated. 
\comment{T: This is the first turn to our contribution! Hence, more explanation (or even re-formatting) could be envisaged!}
%
  \begin{align*}   
   r_T \in \Reachability^{(hyb)}(G,S) \iff r_T \in \Reachability^{(st)}(G,S)\mbox{ and }r_T \in \Reachability^{(top)}(G,S)
  \end{align*}

Applying this hybrid reasoning to the network $G$ consisting of all bold nodes and edges in Fig.~\ref{gra:toy}, 
hybrid minimal solutions would be  $R''_1=\{r_6,r_7,r_{9}\}$ and $R''_2=\{r_6,r_8,r_{9}\}$ \comment{C: same here , and $R''_3=\{r_6,r_7,r_8,r_{9}\}$}. 
They enable to initiate every path of reactions from the seeds $r_5\in\Reachability_{G_i}^{(top)}(\{S_1,S_2\})\mbox{ since }\{A,C\}\subseteq\Sigma_{G}(\{S_1,S_2\})$. 
These solution sets are as well consistent with the steady-state assumption $r_5\in\Reachability_{G_i}^{(st)}(\{S_1,S_2\})$ by balancing the amount of every metabolite.
\comment{C: See if clear}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:


==> tables/optbb_heur1.tex <==
\backslashbox{\core{}}{\prop{}} & 0 & 25 & 50 & 75 & 100\\\hline
0 & \shade{383.3}{600}(133) & \shade{388.51}{600}(133) & \shade{385.73}{600}(135) & \shade{397.2}{600}(136) & \shade{403.31}{600}(139)\\
25 & \shade{387.24}{600}(132) & \shade{385.07}{600}(133) & \shade{382.02}{600}(129) & \shade{386.02}{600}(137) & \shade{402.61}{600}(139)\\
50 & \shade{386.14}{600}(127) & \shade{385.51}{600}(124) & \shade{382.44}{600}(130) & \shade{386.64}{600}(137) & \shade{404.47}{600}(138)\\
75 & \shade{365.92}{600}(127) & \shade{357.03}{600}(125) & \shade{359.55}{600}(131) & \shade{390.26}{600}(137) & \shade{402.3}{600}(140)\\
100 & \shade{377.18}{600}(133) & \shade{380.55}{600}(132) & \shade{383.28}{600}(130) & \shade{384.34}{600}(135) & \shade{402.4}{600}(134)\\


==> tables/optusc_heur1.tex <==
\backslashbox{\core{}}{\prop{}} & 0 & 25 & 50 & 75 & 100\\\hline
0 & \shade{296.6}{600}(100) & \shade{300.23}{600}(103) & \shade{294.72}{600}(103) & \shade{291.65}{600}(101) & \shade{476.06}{600}(201)\\
25 & \shade{297.32}{600}(102) & \shade{296.69}{600}(100) & \shade{294.54}{600}(101) & \shade{297.67}{600}(102) & \shade{474.65}{600}(200)\\
50 & \shade{294.64}{600}(101) & \shade{298.41}{600}(104) & \shade{295.64}{600}(101) & \shade{295.27}{600}(103) & \shade{474.85}{600}(201)\\
75 & \shade{330.12}{600}(128) & \shade{334.66}{600}(130) & \shade{331.19}{600}(129) & \shade{290.98}{600}(102) & \shade{474.89}{600}(200)\\
100 & \shade{311.11}{600}(108) & \shade{310.66}{600}(107) & \shade{327.69}{600}(122) & \shade{489.98}{600}(214) & \shade{474.98}{600}(199)\\

